Distance-based resource quantification for sets of quantum measurements

The advantage that quantum systems provide for certain quantum information processing tasks over their classical counterparts can be quantified within the general framework of resource theories. Certain distance functions between quantum states have successfully been used to quantify resources like entanglement and coherence. Perhaps surprisingly, such a distance-based approach has not been adopted to study resources of quantum measurements, where other geometric quantifiers are used instead. Here, we define distance functions between sets of quantum measurements and show that they naturally induce resource monotones for convex resource theories of measurements. By focusing on a distance based on the diamond norm, we establish a hierarchy of measurement resources and derive analytical bounds on the incompatibility of any set of measurements. We show that these bounds are tight for certain projective measurements based on mutually unbiased bases and identify scenarios where different measurement resources attain the same value when quantified by our resource monotone. Our results provide a general framework to compare distance-based resources for sets of measurements and allow us to obtain limitations on Bell-type experiments.

==> mymath.tex <==
%for process_tom.tex

% ----- new thm environments ------
% \newtheorem{theorem}{Theorem}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{observation}[theorem]{Observation}
% \newtheorem{problem}[theorem]{Problem}

%%%================================================
%%%==============  new commands  =======================
%%%================================================
%------- smaller space in,e.g., $\exp\left(x\right)$
% \let\originalleft\left
% \let\originalright\right
% \renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
% \renewcommand{\right}{\aftergroup\egroup\originalright}
\newcommand{\myleft}{\mathopen{}\mathclose\bgroup\left}
\newcommand{\myright}{\aftergroup\egroup\right}
%%% ------ rm ---------
\newcommand{\e}{\ensuremath\mathrm{e}}
\renewcommand{\i}{\ensuremath\mathrm{i}}
\newcommand{\id}{\ensuremath\mathrm{id}}
\newcommand{\rmd}{\ensuremath\mathrm{d}}
\DeclareMathOperator{\Tr}{Tr}
\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
\DeclareMathOperator{\ran}{ran}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\vecmap}{vec}
\DeclareMathOperator{\Id}{Id}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\spec}{spec}
\DeclareMathOperator{\dist}{dist}
\newcommand{\fro}{\mathrm{F}}
\newcommand{\conv}{\operatorname{conv}}
\DeclareMathOperator{\cone}{\operatorname{cone}}
\DeclareMathOperator{\lin}{\operatorname{lin}}

\DeclareMathOperator{\Pos}{Pos}
\DeclareMathOperator{\CPT}{CPT}
\DeclareMathOperator{\Herm}{Herm}
\DeclareMathOperator{\HT}{HT}%hermiticity and trace preserving
\DeclareMathOperator{\TP}{TP}
%\DeclareMathOperator{\HP}{HP}
\newcommand{\Sym}{\mathrm{Sym}}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Choi}{Choi}

\DeclareMathOperator{\U}{U}%unitary group U(n)
\renewcommand{\O}{\operatorname{O}}%orthogonal group U(n)
\DeclareMathOperator{\SU}{SU}%special unitary group SU(n)

%%% -------- Landau symbols ---------
\DeclareMathOperator{\LandauO}{\mathrm{O}}
\DeclareMathOperator{\tLandauO}{\tilde{\mathrm{O}}}
\DeclareMathOperator{\LandauOmega}{\Omega}


%%% ------- complexity -----------
\usepackage{complexity}%customized
% \newcommand{\NP}{\ComplexityFont{NP}}
\renewcommand{\P}{\ComplexityFont{P}}
\newcommand{\sharpP}{\#\ComplexityFont{P}}


%%% ------ mathbb --------
\newcommand{\CC}{\mathbb{C}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\KK}{\mathbb{K}}% for \RR or \CC
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\1}{\mathbb{1}}
% \newcommand{\EE}{\mathbb{E}}
% \newcommand{\PP}{\mathbb{P}}


%%% ------ mathcal ---------
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\X}{\mc{X}}
\newcommand{\Y}{\mc{Y}}
\newcommand{\V}{\mc{V}}
% \newcommand{\W}{\mc{W}}
\newcommand{\F}{\mc{F}}
% \newcommand{\K}{\mc{K}}
\newcommand{\mcM}{\mc{M}}
\newcommand{\mcL}{\mc{L}}
\newcommand{\mcR}{\mc{R}}
\renewcommand{\H}{\mc{H}}


%%% ------ other ----------
\newcommand{\kw}[1]{\frac{1}{#1}}
\newcommand{\tkw}[1]{\tfrac{1}{#1}}
\newcommand{\argdot}{{\,\cdot\,}}
\renewcommand{\vec}[1]{\boldsymbol{#1}}
\providecommand{\DC}{\operatorname{\mathscr{D}}} %descent cone
\newcommand{\ad}{^\dagger}%symbol for conjugate transpose
\renewcommand{\L}{\operatorname{\mathrm{L}}}%linear operators
\newcommand{\LL}{\operatorname{\mathbb{L}}}%linear maps on operators
% \newcommand{\M}{\operatorname{\mathbb{L}}}
\newcommand{\DM}{\operatorname{\mc{D}}} %density operators
\newcommand{\qqquad}{\qquad\qquad}
\newcommand{\dunion}{\,\dot{\cup}\,}


%%% ------ norms, inner product ----------
\newcommand{\norm}[1]{\left\Vert #1 \right\Vert} %norm with variable height
\newcommand{\normn}[1]{\lVert #1 \rVert} %norm with normalsize height
\newcommand{\normb}[1]{\bigl\Vert #1 \bigr\Vert} %norm with big height
\newcommand{\normB}[1]{\Bigl\Vert #1 \Bigr\Vert} %norm with Big height
\newcommand{\snorm}[1]{\norm{#1}_\infty} %spectral norm  =  (2->2)-norm
\newcommand{\snormn}[1]{\normn{#1}_\infty}
\newcommand{\snormb}[1]{\normb{#1}_\infty}
\newcommand{\snormB}[1]{\normB{#1}_\infty}
\newcommand{\tnorm}[1]{\norm{#1}_{1}} %trace norm
\newcommand{\tnormn}[1]{\normn{#1}_{1}}
\newcommand{\tnormb}[1]{\normb{#1}_{1}}
\newcommand{\TrNorm}[1]{\norm{#1}_{1}} %trace norm
\newcommand{\TrNormn}[1]{\normn{#1}_{1}}
\newcommand{\TrNormb}[1]{\normb{#1}_{1}}
\newcommand{\pNorm}[1]{\norm{#1}_p} %diamond norm
\newcommand{\pNormn}[1]{\normn{#1}_p}
\newcommand{\pNormb}[1]{\normb{#1}_p}
\newcommand{\fnorm}[1]{\norm{#1}_\fro} %Frobenius norm
\newcommand{\fnormn}[1]{\normn{#1}_\fro}
\newcommand{\fnormb}[1]{\normb{#1}_\fro}
%\newcommand{\nnorm}[1]{\norm{#1}_1} %nuclear norm
%\newcommand{\nnormn}[1]{\normn{#1}_1}
%\newcommand{\nnormb}[1]{\normb{#1}_1}
\newcommand{\dnorm}[1]{\norm{#1}_\diamond} %diamond norm
\newcommand{\dnormn}[1]{\normn{#1}_\diamond}
\newcommand{\dnormb}[1]{\normb{#1}_\diamond}
\newcommand{\jnorm}[1]{\norm{#1}_\mysquare} % \jnorm{J(M)}=dim(V)*\dnorm{M}
\newcommand{\jnormn}[1]{\normn{#1}_\mysquare}
\newcommand{\jnormb}[1]{\normb{#1}_\mysquare}
\newcommand{\threenorm}[1]{\lvert\lvert\lvert#1\rvert\rvert\rvert} % ||| . |||
\newcommand{\lTwoNorm}[1]{\norm{#1}_{\ell_2}} %\ell_2 norm
\newcommand{\lTwonormn}[1]{\normn{#1}_{\ell_2}}
\newcommand{\lTwonormb}[1]{\normb{#1}_{\ell_2}}
\newcommand{\lqNorm}[1]{\norm{#1}_{\ell_q}} %\ell_q norm
\newcommand{\lqnormn}[1]{\normn{#1}_{\ell_q}}
\newcommand{\lqnormb}[1]{\normb{#1}_{\ell_q}}
\newcommand{\TwoNorm}[1]{\norm{#1}_{2}} % 2 norm
\newcommand{\TwoNormn}[1]{\normn{#1}_{2}}
\newcommand{\TwoNormb}[1]{\normb{#1}_{2}}

%%% ---- Kets -----
\newcommand{\ket}[1]{\left.\left|{#1}\right.\right\rangle}
\newcommand{\ketn}[1]{| #1 \rangle}
\newcommand{\ketb}[1]{\bigl| #1 \bigr\rangle}
\newcommand{\bra}[1]{\left.\left\langle{#1}\right.\right|}
\newcommand{\bran}[1]{\langle #1 |}
\newcommand{\brab}[1]{\bigl\langle #1 \bigr|}
\newcommand{\braket}[2]{\left\langle #1 \middle| #2 \right\rangle}
\newcommand{\braketn}[2]{\langle #1 \middle| #2 \rangle}
\newcommand{\ketbra}[2]{\ket{#1} \!\! \bra{#2}}
\newcommand{\ketibra}[3]{\ket{#1}_{#2} \!\! \bra{#3}}
\newcommand{\ketbran}[2]{\ketn{#1} \! \bran{#2}}
\newcommand{\ketbrab}[2]{\ketb{#1} \! \brab{#2}}
\newcommand{\sandwich}[3]
  {\left\langle  #1 \right| #2 \left| #3 \right\rangle}
\newcommand{\sandwichb}[3]
  {\bigl\langle  #1 \bigr| #2 \bigl| #3 \bigr\rangle}

%%% ------ specific to this project ----------
\renewcommand{\Pr}{\operatorname{\PP}} 
\newcommand{\Ev}{\operatorname{\EE}} %expectation value
% \newcommand{\A}{\mc{A}} %measurement map
\newcommand{\ev}{e} %error vector
\providecommand{\DC}{\operatorname{\mathscr{D}}} %descent cone
\newcommand{\st}{\mathrm{subject\ to}}
\newcommand{\Haar}{\mathrm{Haar}}
% \newcommand{\minimize}{\mathrm{minimize }}
\DeclareMathOperator*{\minimize}{minimize}
\newcommand{\maximize}{\mathrm{maximize }}
\newcommand{\Span}[1]{\langle #1 \rangle}
\newcommand{\mysquare}{{\protect\scalebox{0.5}{$\square$}}}
%\newcommand{\fd}{f_{\mysquare}}
%\newcommand{\J}{$\mysquare$}
\renewcommand{\r}{_{|r}}
\renewcommand{\c}{_{\neg r}}
\newcommand{\rec}{\mathrm{rec}}
\newcommand{\Toff}{\mathrm{Toff}}
\newcommand{\dep}{\mathrm{dep}}
\newcommand{\eps}{\mathrm{eps}}

\newcommand{\Favg}{F_\mathrm{avg}}
%% ----- algorithmic customisation ------------

% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}


